Segmenting Microcalcifications in Mammograms and its Applications

Microcalcifications are small deposits of calcium that appear in mammograms as bright white specks on the soft tissue background of the breast. Microcalcifications may be a unique indication for Ductal Carcinoma in Situ breast cancer, and therefore their accurate detection is crucial for diagnosis and screening. Manual detection of these tiny calcium residues in mammograms is both time-consuming and error-prone, even for expert radiologists, since these microcalcifications are small and can be easily missed. Existing computerized algorithms for detecting and segmenting microcalcifications tend to suffer from a high false-positive rate, hindering their widespread use. In this paper, we propose an accurate calcification segmentation method using deep learning. We specifically address the challenge of keeping the false positive rate low by suggesting a strategy for focusing the hard pixels in the training phase. Furthermore, our accurate segmentation enables extracting meaningful statistics on clusters of microcalcifications.

==> figs/fig_vis_seg.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\linewidth]{figs/sheba_pred_viz_color.png}
\caption{Our results vs DeepLab V3 results on two Regions Of Interest from Sheba dataset. Note that our output is much more accurate and facilitates the radiologists to extract meaningful statistics as the number of calcifications and their Pleomorphism.\label{fig:sheba_pred_vis}}
\end{figure}  

==> figs/fig_vis_tracking.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{figs/temporal_comparison_3_color.png}
\caption{Accurate segmentation allows to easily compare between mammograms from different times. 
Older on the left. No significant change occurred between the two scans.}
\label{fig:temporal_comparison3} 
\end{figure}  

\begin{figure}
\includegraphics[width=\linewidth]{figs/temporal_comparison_color.png}
\caption{Accurate segmentation allows to easily compare between mammograms from different times.
Although not common, sometimes a reduction in the number of calcifications is observed.}
\label{fig:temporal_comparison} 
\end{figure}

==> figs/sheba_pred_viz.tex <==
\begin{figure}[h!]
    \centering
    % \includegraphics[width=\linewidth]{figs/sheba_pred_viz.png}
    \includegraphics[width=.7\linewidth]{figs/sheba_pred_viz_color.png}
    \caption{Zooming-in to two results from \sheba dataset.}
    \label{fig:sheba_pred_vis} 
\end{figure}

==> figs/table_eval_both.tex <==
% \begin{wraptable}{L}{0.6\linewidth}
% \vspace*{-5mm}
\begin{table}
\centering 
\caption{Quantitative comparison of our method to DeepLabV3 baseline on both Sheba and INbreast datasets. 
%As opposed to InBreast, our dataset contains cases with challenging clusters of microcalcififcations, hence the pronounced gap in performance between our method and the baseline. 
%\rb{Boldface the winner in each category?}\shai{since we are the winners across the board, isn't it just too much?}\rb{No..}
}
\label{tab:eval_both}
\begin{tabular}{|l||c|c||c|c|}
\hline
 & \multicolumn{2}{c||}{ROC AUC} & \multicolumn{2}{c|}{APS} \\
 \cline{2-5}
 &  Sheba &  INbreast &  Sheba &  INbreast \\
 \hline
 \textbf{Ours} & \textbf{0.99} & \textbf{0.98} & \textbf{0.74} & \textbf{0.85} \\
 DeepLabV3 & 0.89 & 0.97 & 0.55 & 0.78 \\
 \hline
\end{tabular}
\end{table}
%\vspace*{-3mm}
%\end{wraptable}


% \begin{tabular}{ccc}
% \begin{tabular}{|c|c|c|}
% \hline
% Method & APS & ROC AUC \\
% \hline
% Our method &  0.74 & 0.99 \\
% DeepLabv3 & 0.55 & 0.89 \\
% \hline
% \end{tabular} & &
% \begin{tabular}{|c|c|c|}
% \hline
% Method & APS & ROC AUC \\
% \hline
% Our method &  0.72 & 0.98 \\
% DeepLabv3 & 0.71 & 0.97 \\
% \hline
% \end{tabular} \\
% \sheba Dataset & & INbreast dataset
% \end{tabular}
% \roee{i calculated the min fpr for tpr=.99 rather than tpr=1. since i assume my manual segmentation is not perfect and i might exceeded the calcification boundaries}

% \shai{describe the different metrics, higher/lower is better? what is the meaning of the measure?} 


% \begin{table}
% \caption{Comparison performance of our method vs other semantic segmentation methods on validation set from INBreast .}
% \label{tab:eval_both}
% \begin{tabular}{cc}

% \begin{tabular}{|c|c|c|c|}
% \hline
% Method & APS & ROC AUC & min FPR for TPR=0.99\\
% \hline
% Our method &  0.74 & 0.99 & 0.07\\
% DeepLabv3 & 0.55 & 0.89 & 0.21\\
% \hline
% \end{tabular} &
% \begin{tabular}{|c|c|c|p{2.4cm}|}
% \hline
% Method & APS & ROC AUC & min FPR for TPR=0.99\\
% \hline
% Our method &  0.72 & 0.98 & 0.08\\
% DeepLabv3 & 0.71 & 0.97 & 0.18\\
% \hline
% \end{tabular}

% \end{tabular}
% \roee{i calculated the min fpr for tpr=.99 rather than tpr=1. since i assume my manual segmentation is not perfect and i might exceeded the calcification boundaries}

% \shai{describe the different metrics, higher/lower is better? what is the meaning of the measure?} 
% \end{table}

==> figs/temporal_comparison.tex <==
\begin{figure}[!t]
    \centering
    % \includegraphics[width=\linewidth]{figs/temporal_comparison.png}
    \includegraphics[width=\linewidth]{figs/temporal_comparison_color.png}

    \caption{Accurate segmentation allows to easily compare between mammograms from different times.}
    \label{fig:temporal_comparison} 
\end{figure}

==> figs/temporal_comparison_3.tex <==
\begin{figure}
    \centering
    % \includegraphics[width=\linewidth]{figs/temporal_comparison_3.png}
    \includegraphics[width=\linewidth]{figs/temporal_comparison_3_color.png}

    \caption{Accurate segmentation allows to easily compare between mammograms from different times (No Change).}
    \label{fig:temporal_comparison3} 
\end{figure}

==> purpose.tex <==
% Microcalcifications are small deposits of calcium that appear in mammograms as bright white specks or dots on the soft
% tissue background (Fig.~\ref{fig:galaxy}). Micro-calcification clusters may be a unique indication for Ductal Carcinoma in Situ breast cancer and thus must be detected. Manual reading of mammograms by radiologists is time consuming, tedious and error-prone since microcalcifications are small and easy to miss. Automated detection methods traditionally suffer from high false-positive rate and therefore not clinically used.
\input{figs/fig1}
Early detection of micro-calcification clusters (see, e.g., Fig~\ref{fig:galaxy}) is important for timely diagnosis of  Ductal Carcinoma in Situ breast cancer.
We address the challenge of accurately segmenting calcifications in high resolution mammograms while keeping low false-positive rate. 
Furthermore, accurate segmentation facilitates the extraction of important statistics such as the number of calcifications in a cluster, their size and variability.
%Pleomorphic features and even to asses temporal change in followup mammograms of a patient.
these statistics, in turn, allow for easier detection of changes in follow-up examinations.


